Equivariant and Invariant Grounding for Video Question Answering

Video Question Answering (VideoQA) is the task of answering the natural language questions about a video. Producing an answer requires understanding the interplay across visual scenes in video and linguistic semantics in question. However, most leading VideoQA models work as black boxes, which make the visual-linguistic alignment behind the answering process obscure. Such black-box nature calls for visual explainability that reveals ``What part of the video should the model look at to answer the question?''. Only a few works present the visual explanations in a post-hoc fashion, which emulates the target model's answering process via an additional method. Nonetheless, the emulation struggles to faithfully exhibit the visual-linguistic alignment during answering. Instead of post-hoc explainability, we focus on intrinsic interpretability to make the answering process transparent. At its core is grounding the question-critical cues as the causal scene to yield answers, while rolling out the question-irrelevant information as the environment scene. Taking a causal look at VideoQA, we devise a self-interpretable framework, Equivariant and Invariant Grounding for Interpretable VideoQA (EIGV). Specifically, the equivariant grounding encourages the answering to be sensitive to the semantic changes in the causal scene and question; in contrast, the invariant grounding enforces the answering to be insensitive to the changes in the environment scene. By imposing them on the answering process, EIGV is able to distinguish the causal scene from the environment information, and explicitly present the visual-linguistic alignment. Extensive experiments on three benchmark datasets justify the superiority of EIGV in terms of accuracy and visual interpretability over the leading baselines.

==> backup/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}


% 1.videoQA overview-----------------------------------------
% 第一段介绍背景：
% 一句话介绍VideoQA的重要性；
% 一句话介绍VideoQA的task；
% 然后引出现有VideoQA models都是black-box的困扰；
% 2-3句话介绍black-box的坏处是啥。

\wx{Video Question Answering (VideoQA) \cite{fan2019heterogeneous} is a keystone in interactive AI, such as vision-language navigation and communication systems.
It aims to answer the natural language question based on the video content.}


In pursuance of interactive AI, Video Question Answering (VideoQA) \cite{fan2019heterogeneous} serves as a keystone in abridging human cognition and machine intelligence, whose goal is to answer the natural language question based on the video content.   
%
Nourished by its multi-modal nature, VideoQA \textit{per se} has relished an overwhelming expansion in model design, which either fosters the vision-language alignment \cite{jiang2020reasoning,park2021bridge} or revisit the visual input structure \cite{le2021hierarchical,dang2021hierarchical}.
%
Albeit their sterling performance, existing solutions are usually expressed as black boxes, where the intrinsic rationale --- how to identify the question-responsive visual elements, is still clouded from our intuition. 
%
As a result, such opaqueness certainly raises reliability concern when the model is deployed in the real-word application, such as \ie intelligent surveillant assistant or more generally, an out-of-distribution test setting.

% More frustratingly, the system gives
% no hint about which part of such systems is the
% culprit for a wrong answer

\begin{figure}[t]
\centering
\includegraphics[scale=0.53]{fig/f1.pdf}
\caption{Illustration of causal-equivariant and environment-invariant principle, where $x$ is the input video-question pair, $f$ is a map from input space to answer space, $T$ is a transformation operator that applies to both input and answer space}.
% (\textcolor[rgb]{0,0.5,0}{Green}: causal-equivarince; \textcolor[rgb]{0.03,0.27,0.49}{Navy}: complement-invariance)}
\vspace{-5pt}
\label{fig:overview}
\end{figure}


% 2.problem of interpretable-------------------------------
% 第二段介绍explainability/interpretability in VideoQA：
% 一句话描述：对于black-box nature的concerns，explainability in VideoQA非常重要；
% 一句话描述：explainability in VideoQA是要回答什么问题：which part of the video should the model look at to answer the question?
% 然后说明现在都是post-hoc explanations，这里要点出来post-hoc的基本概念是啥；然后一两句话介绍post-hoc为啥有缺陷。

Trust concern on the black-box nature of existing methods calls upon a comprehensive study on model interpretability, \ie how they arrive at a specific prediction. 
%
In the context of the VideoQA, a favorable interpretation ought to answer the million-dollar question "which part of the video should the model look at to answer the question?" 
%
Despite the necessity, the explainability of the current design still dwells on the post-hoc paradigm \cite{gao2018motionappearance,DBLP:conf/iccv/Liu0WL21,10.1145/3474085.3475620}, where interpretations are approximated by extracting a salience pattern from the trained predictive model without any inductive knowledge ( \eg visualize attention weight).
%
Unfortunately, the visual justification via the post-hoc method is fragile against input perturbations, since some artifacts can be easily captured as explanations instead of genuine knowledge from the data \cite{DBLP:conf/ijcai/LaugelLMRD19}. As a result, peeking through output (\ie Grad-CAM \cite{DBLP:conf/iccv/SelvarajuCDVPB17}) is implicit and cannot faithful reveals how machine leverage the multi-modal information, which left our million-dollar concern unaddressed.

% which is fragile against input perturbations, and less instructive to the predictive mechanism. 


% In addition, it is debatable whether attention mechanisms are indeed explanations (Wiegreffe and Pinter, 2019; Jain and Wallace, 2019). M

% Worse still, overwhelming computational power has provoked the model complexity with billions of parameters, which, as a seed of distrust, shadowed the model's transparency along with our faith. 
%


% 3.partition the video to get interpretation ------------
% 第三段讲我们要研究的内容：
% 一句话介绍我们关注intrinsic interpretability，但是研究的人很少；
% 一句话描述我们的self-interpretable问题是“which part of the video is critical/causal to answering the question?”
% 然后引出我们要把visual scenes分成两部分一部分是causal scene，一部分是environmental scenes：分别介绍这两个具有啥子semantics。

Clearly, inferring a reliable rationale requires intrinsic interpretability to illuminate the reasoning insight. 
%
However essential, a self-interpretable VideoQA explainer that reveals such intrinsic prediction mechanism is until-now lacking.
%
To fill this gap, we get inspiration from \textit{causal theory} \cite{pearl2016causal} and capture such self-interpretability by answering the question of gold --- ``which part of the video is critical/causal to answering the question?'' 
% 
Concretely, we aim to find the causal part of input video on-the-fly that preserves the maximum visual information toward the question, whose discovery will justify the prediction and encourage the generalization.
%
Following this essence, one straightforward realization is to empower the model with discernment that grounds the visual scene into two segments: 
(1) \textbf{causal scene} that retains the question-critical video content and preserves all the relevant information about the target answer, which naturally serves as interpretation for the prediction; (2) \textbf{environment scene} that holds answer-irrelevant environment information of input video. 

% To the best of our knowledge, a self-interpretable VideoQA explainer that reveals the intrinsic prediction mechanism is critical to trustworthy videoQA but until-now lacking.
%

% Clearly, inferring a reliable answer requires a grounding rationale of the prediction, \ie to answer the million-dollar question "which part of the video scene should  be looking at?". 
%
% Inspired by the information bottleneck, which tends to reduce the overload of information processing \cite{DBLP:conf/iclr/SaxeBDAKTC18}, we aim to find the causal for input video that preserves the maximum visual information toward the question, whose discovery will justify the prediction and increase the generalization. 

%
% Following this essence, one straightforward solution is to empower the model with discernment that splits the visual scene into two segments: 
% (1) \textbf{causal scene} that retains the question-critical video content and preserving all the relevant information about the target answer, which naturally serves as interpretation for the prediction; (2) \textbf{environment scene} that holds answer-irrelevant environment information of input video. 


% 4.euiqvariant and invariant -------------------------------
% 要突出的是grounding，title中是Equivariant and invariant grounding，所以要让这些关键词尽早的出现。
% 这个例子融入到下面的Causal-Equivariance和Environmental-Invariance中去。
%
Discovering causal scene without fine-grained supervision is a luxury for VideoQA. Gazed upon the reasoning process, we argue the crux of this problem is to amplify the connection between the causal scene and the answer, while blocking the effect of the environment. 
%
Following this line, we put forward two principles to guide the grounding of the rationale.
%
% Following this line, we put forward \textit{Equivariance} and \textit{Invariance} principles to guide the grounding process.
% %
% Specifically, equivariance extends the model's sensitivity towards the a transformation $T$ on input $x$. Invariance, quite the contrary, inhibits the sensitivity and block model from input transformation. In light of this, the discovery of a stable rationale implies two requirements on the partition:
%
\begin{itemize}[leftmargin=*]
    \item \textbf{Causal-euqivariance.} 
    In essence, transformation on the causal scene should cause the parallel change on the representation manifold. By introspecting ``How would the predictive answer vary if the causal scenes change?'', the grounding mechanism is aware of the transformations and thus maintains the predictive interpretation.
    %
    As exemplified in Figure \ref{fig:overview}, equivariance implies that transformation applied to answer-critic information (\ie causal scene and question) should set off an equivariant semantic change in answer space.
    %
    Correspondingly, a cautious formulation of such co-variation should help the model pinpoint the 'girl-on-horse' scene as a grounding rationale for ``ride''.
    
    \item \textbf{Environment-invariance.} 
    % 是它不符合human cognition以及它会产生spurious correlation
    On the ground of the prophet, permutation on environment scene should be invariant to predictive answer, since environment implies no impact to the predictive answer except spurious correlation, comprising it as rationale runs counter to the human cognition. 
    % On ground of the prophet, the predictive answer is invariant against permutation on environment scene, as it does not contribute to the reasoning mechanism or interpretation.
    %
    Consider the example in Figure \ref{fig:overview} again, since an environment like ``landscape'' provides no evidence toward the answer ``ride'', its corresponding transformation should reflect a homogeneity in the answer space. The invariance principle epitomizes such assumption by ruling a transformation that is in-vary to answer permutation.
\end{itemize}


%5.overall idea ------------------------------------------------------------------
% Aspiring to capture grounding rationale, we formalize a model-agnostic learning framework, Equivariant and Invariant Grounding for Interpretable VideoQA (EIV), 
% %
% by asking the question ``what and how transformation should the model be equivariant or invariant to?'' 
% %
% Different from the previous effort that design supervised proxy task for geometric transformation \cite{DBLP:conf/iccv/ChengSM21}, 
% % we adopted philosophy of causal intervention and design a saliency-aware temporal mix method for the video input, and impose 
% we answer the ``what'' question by adopting the philosophy of causality \cite{pearl2009causal} and configure transformation as causal intervention operation that imposes scene-aware mixup \cite{DBLP:conf/iclr/ZhangCDL18} on the multi-modal input.
% %
% As for the question of how, we present a unified view of equivariant and invariant principles via the lens of temporal self-supervised learning, where the contrastive counterparts are bred through a disruption on the causal scene, environment scene as well as vision-language alignment.

% where the contrastive counterparts are bred through a disruption on the causal and environment scene, respectively.

% implemetation ----------------------------------------------
% 这一段的写作逻辑应该是如何实现equivariant、invariant principles的；可以不用follow IGV的写法；

% 可以这么组织：
% 一句话介绍三个modules；
% 然后如何用这三个modules来实现两个principle的：首先用grouidng indicator去roughly partition videos into two parts：causal and environmental scenes；然后基于这两部分引入causal-equivariance：利用interventer对于causal scenes做interventions，期望answer部分产生相对应的变化；利用interventer对于environmental scenes做interventions，期待这部分不会对于answering产生影响。
In light of the proposed princes, we formalize EIGV (\underline{E}quivariant and \underline{I}nvariant \underline{G}rounding for Interpretable \underline{V}ideoQA),
a model-agnostic explainer to capture the stable visual rationale VideoQA models.
% 一句话介绍三个modules；
Specifically, EGV absorbs three modules in addition to the backbone VideoQA model: a grounding indicator, an intervener, and a disruptor. 
%
%grounding indicator
In particular, the grounding indicator learns to separate the causal scenes as the interpretation and leave the rest as the environment. 
%
% causal-equivariance
Then, for the causal scene of interest, an intervener imposes the equivariance principle via a convex combination of two data points, while anticipating a corresponding change in the answer space.  
%
% environment-invariance
As for the environment counterpart, the invariant principle is realized using a similar intervener, but expecting an unchanged answer.
% %
% Noticeably, since mixing environment does not affect the reasoning dynamics, the answer is modified with the same ratio as the causal scene but independent to environmental one. 
%
% By capturing the equivariance from the answer to the causal scene and the invariance to environment, the model perceives a faithful interpretation that preserves the predictive mechanism.
%
On top of the intervened video, we present a unified view of equivariant and invariant principles via the lens of temporal self-supervised learning. 
%
Concretely, a disruptor substitutes the environment and causal scene with the stratification sampled from a memory bank (a collection of other training videos) to constitute the contrastive twins, respectively. 
%
% To fortify visual-question pair-wise cohesiveness, we also develops alternatives in addition to visual negatives by disrupting the visual-question coupling.
%
In addition to the visual negatives, we also develop alternatives by disrupting the visual-question coupling, to fortify their pair-wise cohesiveness.

% where the contrastive counterparts are bred through a disruption on the causal scene, environment scene as well as vision-language alignment.

% On top of the intervened video, the disruptor substitutes the complement scene with the stratification sampled from a memory bank (a collection of other training videos) and constitutes the “counterfactual video” as the positive sample.
% Likewise, the negative sample is constructed via replacement on the causal scene. 
% %
% In addition to the visual negatives that ``disrupt'' the causal scene, the disruptor also develops alternatives by disrupting the visual-question coupling, to fortify their pair-wise cohesiveness.
% 
After acquiring anchor representation alongside its contrastive twins, the auxiliary contrastive objective reveals the discriminative representation purely from the scene of interest, thus fostering the robustness of interpretation.

Briefly put, our contributions are: 
\begin{itemize}[leftmargin=*]
    \item We propose EGV, a model-agnostic VideoQA explainer that captures the intrinsic causal pattern in a self-interpretable manner.
    
    \item We investigate the soundness of grounding rationale by posing the equivariant-invariant principle on visual grounding and realize it via the causal instrument.
    
    \item We justify the superiority of EGV on three popular benchmark datasets (\ie MSVD-QA \cite{DBLP:conf/mm/XuZX0Z0Z17}, MSRVTT-QA \cite{DBLP:conf/mm/XuZX0Z0Z17},  NExT-QA \cite{DBLP:conf/cvpr/XiaoSYC21}) with extensive experiments, where our design outmatches all the state-of-the-art models.
\end{itemize}















==> backup/1_intro_new.tex <==
\section{Introduction}
\label{sec:introduction}


% 1.videoQA overview-----------------------------------------
% 第一段介绍背景：
% 一句话介绍VideoQA的重要性；
% 一句话介绍VideoQA的task；
% 然后引出现有VideoQA models都是black-box的困扰；
% 2-3句话介绍black-box的坏处是啥。

\wx{Video Question Answering (VideoQA) \cite{fan2019heterogeneous} is a keystone in interactive AI, such as vision-language navigation and communication systems.
It aims to answer the natural language question based on the video content.
Nourished by the multi-modal nature, VideoQA \emph{per se} has relished an expansion in the model design, which spans from fostering the vision-language alignment \cite{jiang2020reasoning,park2021bridge} to revisiting the visual input structure \cite{le2021hierarchical,dang2021hierarchical}.
However, existing VideoQA models usually work as black boxes, which fail to exhibit the working mechanism behind the predictions and hardly reveal ``What knowledge should the model use to answer the question about the video?''.
% However, existing VideoQA models usually work as black boxes, which fail to exhibit the intrinsic rationale behind the predictions and hardly answer ``What knowledge should the model use to answer the question about the video?''.
As a result, the black-box nature causes concern for the model reliability and hinders the model deployment, especially in applications on safety and security.

}

% More frustratingly, the system gives
% no hint about which part of such systems is the
% culprit for a wrong answer

\begin{figure}[t]
\centering
\includegraphics[scale=0.47]{fig/f1.pdf}
\caption{Illustration of causal-equivariant and environment-invariant principles, where $C,E$ are the causal and environment of input video, $f_{\hat{A}}$ is a map from input space to answer space, $T_{\epsilon}$ and $T_{\iota}$ are transformations (instantiated as a mixture of two data points) that applies to causal and non-causal factors, respectively.}
% (\textcolor[rgb]{0,0.5,0}{Green}: causal-equivarince; \textcolor[rgb]{0.03,0.27,0.49}{Navy}: complement-invariance)}
\vspace{-18pt}
\label{fig:overview}
\end{figure}


% 2.problem of interpretable-------------------------------
% 第二段介绍explainability/interpretability in VideoQA：
% 一句话描述：对于black-box nature的concerns，explainability in VideoQA非常重要；
% 一句话描述：explainability in VideoQA是要回答什么问题：which part of the video should the model look at to answer the question?
% 然后说明现在都是post-hoc explanations，这里要点出来post-hoc的基本概念是啥；然后一两句话介绍post-hoc为啥有缺陷。


% \wx{
% The concern on the black-box nature calls for explainability of VideoQA models.
% Here we focus on visual-explainability \cite{CSS,DBLP:conf/ijcai/RossHD17}, aiming to answer ``Which part of the video should the model look at to answer the question?''.
% It inspires us to ground a subset of visual scenes --- rationale --- which are the right reasons for the right answering \cite{DBLP:conf/ijcai/RossHD17}.
% Towards this end, the current studies \cite{gao2018motionappearance,DBLP:conf/iccv/Liu0WL21,10.1145/3474085.3475620} dwell on the ``learning to attend'' paradigm \cite{DBLP:conf/nips/VaswaniSPUJGKP17,DBLP:conf/icml/XuBKCCSZB15}, which uses the attention mechanism to identify some informative scenes as the explanation.
% To optimize the attention mechanism, empirical risk minimization (ERM)
% }


\wx{
The concern on the black-box nature calls for explainability of VideoQA models.
Here we focus on visual-explainability \cite{CSS,DBLP:conf/ijcai/RossHD17}, aiming to reveal ``Which part of the video should the model look at to answer the question?''.
It requires us to find a subset of visual scenes --- rationale --- which are the right reasons for the right answering \cite{DBLP:conf/ijcai/RossHD17}.
Taking Figure \ref{fig:overview} as an example, when answering the question ``What is the girl doing?'', the rationale should focus on the ``girl-riding on-horse'' scene in the first two clips.
% Towards this end, there are two prevalent paradigms: post-hoc explainability, intrinsic interpretability.
Towards this end, the current studies \cite{gao2018motionappearance,DBLP:conf/iccv/Liu0WL21,10.1145/3474085.3475620} dwell mainly on the paradigm of \textbf{post-hoc explainability} \cite{LIME,DBLP:conf/iccv/SelvarajuCDVPB17}, which distributes the target model's predicted answer to the input visual features via an additional explainer method.
They visualize the attention weights or gradient-like signals about the visual features, and then identify a salient pattern as the rationale.
However, post-hoc explainability has several major limitations:
(1) It fails to make the target model intrinsically interpretable \cite{DBLP:conf/cvpr/YangZQ021,DBLP:conf/iccv/WangZSZ21}, only approximating the decision-making process of the model.
As a result, the identified rationale cannot faithfully reveal how the model leverages the multi-modal information.
(2) Such visual inspections are fragile against input perturbations, since some artifacts can be easily captured as explanations instead of genuine knowledge from the data \cite{DBLP:conf/ijcai/LaugelLMRD19,slack2020fooling,heo2019fooling,ghorbani2019interpretation}.
}


% Trust concern on the black-box nature of existing methods calls upon a comprehensive study on model interpretability, \ie how they arrive at a specific prediction. 
% %
% In the context of the VideoQA, a favorable interpretation ought to answer the million-dollar question "which part of the video should the model look at to answer the question?" 
% %
% Despite the necessity, the explainability of the current design still dwells on the post-hoc paradigm \cite{gao2018motionappearance,DBLP:conf/iccv/Liu0WL21,10.1145/3474085.3475620}, where interpretations are approximated by extracting a salience pattern from the trained predictive model without any inductive knowledge ( \eg visualize attention weight).
% %
% Unfortunately, the visual justification via the post-hoc method is fragile against input perturbations, since some artifacts can be easily captured as explanations instead of genuine knowledge from the data \cite{DBLP:conf/ijcai/LaugelLMRD19,slack2020fooling,heo2019fooling,ghorbani2019interpretation}. As a result, peeking through output (\za{\eg LIME \cite{LIME}}, Grad-CAM \cite{DBLP:conf/iccv/SelvarajuCDVPB17}) cannot faithfully reveal how machine leverage the multi-modal information, which left our million-dollar concern unaddressed.

% which is fragile against input perturbations, and less instructive to the predictive mechanism. 


% In addition, it is debatable whether attention mechanisms are indeed explanations (Wiegreffe and Pinter, 2019; Jain and Wallace, 2019). M

% Worse still, overwhelming computational power has provoked the model complexity with billions of parameters, which, as a seed of distrust, shadowed the model's transparency along with our faith. 
%


% 3.partition the video to get interpretation ------------
% 第三段讲我们要研究的内容：
% 一句话介绍我们关注intrinsic interpretability，但是研究的人很少；
% 一句话描述我们的self-interpretable问题是“which part of the video is critical/causal to answering the question?”
% 然后引出我们要把visual scenes分成两部分一部分是causal scene，一部分是environmental scenes：分别介绍这两个具有啥子semantics。

\wx{The limitations of post-ho explainability inspire us to explore the paradigm of \textbf{intrinsic interpretability} \cite{ghorbani2019interpretation}, which implants a rationalization module into the model to make the decision-making process transparent.
Surprisingly, intrinsic interpretability of VideoQA models is until-now lacking but our focus in this work.
To fill the void, we draw on \textbf{causal theory} \cite{pearl2016causal,pearl2009causal} to formulate the interpretability task as answering ``Which part of the video is critical/causal to answering the question?''.
Concretely, we aim to identify the causal component of input video on-the-fly, which holds the question-response information and filters the question-irrelevant cues out.
Following this essence, one straightforward realization is to ground the input video into two segments:
(1) \textbf{causal scene}, which retains the question-critical visual content and sufficiently approaches the answer, thus naturally serving as the rationale;
(2) \textbf{environment scene}, which holds the question-irrelevant visual content and can be seen as the rationale's complement.
}



% 4.euiqvariant and invariant -------------------------------
% 要突出的是grounding，title中是Equivariant and invariant grounding，所以要让这些关键词尽早的出现。
% 这个例子融入到下面的Causal-Equivariance和Environmental-Invariance中去。
%
\wx{However, discovering causal scene without the supervision of ground-truth rationale is challenging.
With a causal look at the reasoning process (\cf Section \ref{sec:causal-view}), we argue the crux of intrinsic interpretability is to amplify the connection between the causal scene and the answer, while blocking the non-causal effect of the environment scene.
Following this line, we propose two principles to guide the grounding of the rationale:}
\begin{itemize}[leftmargin=*]
    \item \textbf{Causal-Equivariance.}
    \wx{By ``equivariance'', we mean that answering should be sensitive to the semantic changes on the causal scene and question (termed E-intervention), \eg any change on the causal scene and question should be faithfully reflected on the predicted answer. For example, the ``girl-riding on-horse'' and \lyc{``man-surfing in-ocean''} scenes are the oracle rationales of ``What is the girl doing?'' and ``What is the man doing?'', respectively. The intervention applied on the input (\ie mixing the ``girl-riding on-horse'' and \lyc{``man-surfing in-ocean''} scene, and combining two questions as ``What is the girl doing? What is the man doing?'') should set off an equivariant change in the answer (\ie changing from ``Ride'' to ``Ride+\lyc{Surf}'').
    }
    
    
    % In essence, transformation on the causal scene should cause the parallel change on the representation manifold. By introspecting ``How would the predictive answer vary if the causal scenes change?'', the grounding mechanism is aware of the transformations and thus maintains the predictive interpretation.
    % %
    % As exemplified in Figure \ref{fig:overview}, equivariance implies that transformation applied to question-critic information (\ie causal scene and question) should set off an equivariant semantic change in answer space.
    % %
    % Correspondingly, a cautious formulation of such co-variation should help the model pinpoint the 'girl-on-horse' scene as a grounding rationale for ``ride''.
    
    \item \textbf{Environment-Invariance.}
    \wx{By ``invariance'', we mean that answering should be insensitive to the changes in the environment (termed I-intervention), conditioning on the causal scene and question.
    Considering Figure \ref{fig:overview} again, the intervention applied on the environment (\ie mixing the ``meadow'' and \lyc{``ocean''} scenes) implies no impact towards answering ``What is the girl doing?'', reflecting a homogeneity in the answer space.
    }

    
    % % 是它不符合human cognition以及它会产生spurious correlation
    % On the ground of the prophet, permutation on environment scene should be invariant to predictive answer, since environment implies no impact to the predictive answer except spurious correlation, comprising it as rationale runs counter to the human cognition. 
    % % On ground of the prophet, the predictive answer is invariant against permutation on environment scene, as it does not contribute to the reasoning mechanism or interpretation.
    % %
    % Consider the example in Figure \ref{fig:overview} again, since an environment like ``landscape'' provides no evidence toward the answer ``ride'', its corresponding transformation should reflect a homogeneity in the answer space. The invariance principle epitomizes such assumption by ruling a transformation that is in-vary to answer permutation.
\end{itemize}


%5.overall idea ------------------------------------------------------------------
% Aspiring to capture grounding rationale, we formalize a model-agnostic learning framework, Equivariant and Invariant Grounding for Interpretable VideoQA (EIV), 
% %
% by asking the question ``what and how transformation should the model be equivariant or invariant to?'' 
% %
% Different from the previous effort that design supervised proxy task for geometric transformation \cite{DBLP:conf/iccv/ChengSM21}, 
% % we adopted philosophy of causal intervention and design a saliency-aware temporal mix method for the video input, and impose 
% we answer the ``what'' question by adopting the philosophy of causality \cite{pearl2009causal} and configure transformation as causal intervention operation that imposes scene-aware mixup \cite{DBLP:conf/iclr/ZhangCDL18} on the multi-modal input.
% %
% As for the question of how, we present a unified view of equivariant and invariant principles via the lens of temporal self-supervised learning, where the contrastive counterparts are bred through a disruption on the causal scene, environment scene as well as vision-language alignment.

% where the contrastive counterparts are bred through a disruption on the causal and environment scene, respectively.

% implemetation ----------------------------------------------
% 这一段的写作逻辑应该是如何实现equivariant、invariant principles的；可以不用follow IGV的写法；

% 可以这么组织：
% 一句话介绍三个modules；
% 然后如何用这三个modules来实现两个principle的：首先用grouidng indicator去roughly partition videos into two parts：causal and environmental scenes；然后基于这两部分引入causal-equivariance：利用interventer对于causal scenes做interventions，期望answer部分产生相对应的变化；利用interventer对于environmental scenes做interventions，期待这部分不会对于answering产生影响。

\wx{To impose these two principles for intrinsic interpretability, we propose a new framework, \underline{E}quivariant and \underline{I}nvariant \underline{G}rounding for Interpretable \underline{V}ideoQA (\textbf{EIGV}).
EIGV equips the VideoQA backbone model with three additional modules:
a grounding indicator, an intervener, and a disruptor.
First, the grounding indicator learns to attend the causal scene based on the input question, while leaving the rest as the environment.
% However, this grounding only roughly estimates the oracle partition of causal and environment scenes.
Then, the intervener parameterizes these principles to guide the grounding.
Specifically, towards the causal-equivariance principle, it conducts the E-intervention on the causal scene and question --- that is, mix them with the counterparts from another video-question pair --- and encourages the answering to be anticipated accordingly.
Towards the environment-invariance principle, when leaving the causal scene and question untouched, it applies the I-intervention on the environment --- that is, mix it with the environmental stratification of a memory bank --- and enforces the predicted answer to be invariant.
On the top of intervened video-question pairs, the disruptor constructs the contrastive twins.
}


% In light of the proposed princes, we formalize EIGV (\underline{E}quivariant and \underline{I}nvariant \underline{G}rounding for Interpretable \underline{V}ideoQA),
% a model-agnostic explainer to capture the stable visual rationale VideoQA models.
% % 一句话介绍三个modules；
% Specifically, EGV absorbs three modules in addition to the backbone VideoQA model: a grounding indicator, an intervener, and a disruptor. 
%
%grounding indicator
In particular, the grounding indicator learns to separate the causal scenes as the interpretation and leave the rest as the environment. 
%
% causal-equivariance
Then, for the causal scene of interest, an intervener imposes the equivariance principle via a convex combination of two data points, while anticipating a corresponding change in the answer space.  
%
% environment-invariance
As for the environment counterpart, the invariant principle is realized using a similar intervener, but expecting an unchanged answer.
% %
% Noticeably, since mixing environment does not affect the reasoning dynamics, the answer is modified with the same ratio as the causal scene but independent to environmental one. 
%
% By capturing the equivariance from the answer to the causal scene and the invariance to environment, the model perceives a faithful interpretation that preserves the predictive mechanism.
%
On top of the intervened video, we present a unified view of equivariant and invariant principles via the lens of temporal self-supervised learning. 
%
Concretely, a disruptor substitutes the environment and causal scene with the stratification sampled from a memory bank (a collection of other training videos) to constitute the contrastive twins, respectively. 
%
% To fortify visual-question pair-wise cohesiveness, we also develops alternatives in addition to visual negatives by disrupting the visual-question coupling.
%
In addition to the visual negatives, we also develop alternatives by disrupting the visual-question coupling, to fortify their pair-wise cohesiveness.

% where the contrastive counterparts are bred through a disruption on the causal scene, environment scene as well as vision-language alignment.

% On top of the intervened video, the disruptor substitutes the complement scene with the stratification sampled from a memory bank (a collection of other training videos) and constitutes the “counterfactual video” as the positive sample.
% Likewise, the negative sample is constructed via replacement on the causal scene. 
% %
% In addition to the visual negatives that ``disrupt'' the causal scene, the disruptor also develops alternatives by disrupting the visual-question coupling, to fortify their pair-wise cohesiveness.
% 
After acquiring anchor representation alongside its contrastive twins, the auxiliary contrastive objective reveals the discriminative representation purely from the scene of interest, thus fostering the robustness of interpretation.

Briefly put, our contributions are: 
\begin{itemize}[leftmargin=*]
    \item We propose EGV, a model-agnostic VideoQA explainer that captures the intrinsic causal pattern in a self-interpretable manner.
    
    \item We investigate the soundness of grounding rationale by posing the equivariant-invariant principle on visual grounding and realize it via the causal instrument.
    
    \item We justify the superiority of EGV on three popular benchmark datasets (\ie MSVD-QA \cite{DBLP:conf/mm/XuZX0Z0Z17}, MSRVTT-QA \cite{DBLP:conf/mm/XuZX0Z0Z17},  NExT-QA \cite{DBLP:conf/cvpr/XiaoSYC21}) with extensive experiments, where our design outmatches all the state-of-the-art models.
\end{itemize}















==> backup/1_intro_v0.tex <==
\section{Introduction}
\label{sec:introduction}


% 1.videoQA overview-----------------------------------------
In name of the interactive AI, Video Question Answering (VideoQA) \cite{fan2019heterogeneous} has relished a overwhelming expansion in various domains, such as vision-language navigation and communication systems. 
%
To answer the natural language question based on the video content, the task \textit{per se} has bred multi-modal nature in its process of reasoning, which demands thorough comprehension across visual content and linguistic semantics.

% %
% Aiming to answer the natural language question based on the video content, Video Question Answering (VideoQA) \cite{fan2019heterogeneous} 
% has witnessed aggressive expansion in various domains, such as vision-language navigation and communication systems.
% To make the task intriguing, the multi-modal nature of VideoQA has bred interactive AI in its reasoning, which demands thorough comprehension across visual scenes and linguistic semantics.
%
% In this regard, various VidoeQA model realizes their excellence via a common paradigm of two modules:
% (1) \textit{video-question encoder} encapsulates the video content and the question semantics to representations;
% and (2) \textit{answer decoder} exploits the multi-modal representations to model the vision-language interaction and generate an answer. 

\begin{figure}[t]
\centering
\includegraphics[scale=0.53]{fig/f1.pdf}
\caption{Illustration of causal-equivariant and environment-invariant principle, where $x$ is the model input, $f$ is a map from input space to answer space, $T$ is a transformation operator that applies to both input and answer space}.
% (\textcolor[rgb]{0,0.5,0}{Green}: causal-equivarince; \textcolor[rgb]{0.03,0.27,0.49}{Navy}: complement-invariance)}
\vspace{-5pt}
\label{fig:overview}
\end{figure}

% 2.problem of interpretable-------------------------------
Albeit the sterling performance, existing efforts usually express their reasoning mechanisms as black boxes. Unfortunately, peeping through their output does not reveal how machine leverage the multi-modal information, which refrains human intuition from machine intelligence and repels the nature of interactive AI. 
%the explanation of black-box models can provide insights into the relationship between input and output, thereby improving model design.
%shed light on model design
Worse still, overwhelming computational power has provoked the model complexity with billions of parameters, which, as a seed of distrust, shadowed the model's transparency along with our faith. 
%
Despite the necessity, the explainability of the current design still dwells on post-hoc visualization \cite{gao2018motionappearance,DBLP:conf/iccv/Liu0WL21,10.1145/3474085.3475620}, which is fragile against input perturbations, and less instructive to the predictive mechanism. 
%
% Clearly, inferring a reliable answer requires grounding rationale of the prediction, \ieto answer the million dollar question "which part of the video scene should be look at to answer the question". 
%
To the best of our knowledge, a self-interpretable VideoQA explainer that reveals the intrinsic prediction mechanism is critical to trustworthy videoQA but until-now lacking. 

% 3.partition the video to get interpretation ------------
Clearly, inferring a reliable answer requires a grounding rationale of the prediction, \ie to answer the million-dollar question "which part of the video scene should  be looking at?". 
%
Inspired by the information bottleneck, which tends to reduce the overload of information processing \cite{DBLP:conf/iclr/SaxeBDAKTC18}, we aim to find a shortcode for input video that preserves the maximum visual information toward the question, whose discovery will justify the prediction and increase the generalization. 
%
% Intuitively, filtering out task-irrelevant information reduces the overload of information processing, which naturally makes the representation more controllable.
%
Following this essence, one straightforward solution is to empower the model with discernment that splits the visual scene into two segments: 
(1) \textbf{causal scene} that retains the question-critical video content and preserving all the relevant information about the target answer, which naturally serves as interpretation for the prediction; (2) \textbf{environment scene} that holds answer-irrelevant environmental information of input video. 

% 4.euiqvariant and invariant for robust interpretation ---------------------------
% Modifying model's sensitivity to a certain transformation can have a substantial effect on the robustness of representation \cite{DBLP:journals/corr/abs-2111-00899}.
% %
% On top of the partition, one natural notion to acquire robust interpretation is making model sensitive to transformation of casual sense, while insensitive to transformation of complement sense.
% %
% Such philosophy of sensitivity is captured by the mathematical concept of equivariance and invariance: for a input$x$ and non-parametric transformation $T$, a encoder $f(.)$ is equivariant to $T$, if $∀x : f(T(x)) = T(f(x))$ ; Likewise, invariance is defined as $∀x : f(T(x)) = f(x)$.
% Specifically, the discovery of stable rationale implies two requirements on the partition:

%%%%%%
% Discovering  causal scene and answer is a luxury for videoQA without fine-grained supervision. 
Discovering causal scene without fine-grained supervision is a luxury for videoQA. Gazed upon the reasoning process, we argue crux of this problem is to amplify the connection between the causal scene and answer, while blocking the effect of environment. Following this line, we put forward \textit{Equivariance} and \textit{Invariance} principles to guide the partition learning.
% we borrow the mathematical concept of equivariance and invariance.
As shown in Figure \ref{fig:overview}, equivariance extends the model's sensitivity towards the a transformation $T$ on input $x$. Invariance, quite the contrary, inhibits the sensitivity and block model from input transformation. In light of this, the discovery of a stable rationale implies two requirements on the partition:
%
\begin{itemize}[leftmargin=*]
    \item \textbf{Causal-euqivariance.} In essence, transformation on the causal scene should cause the parallel change on the representation manifold. By introspecting ``How would the predictive answer vary if the causal scenes change?'', the grounding mechanism is aware of the transformations and thus maintains the predictive interpretation.
    In Figure \ref{fig:overview}, the euqivariance is exemplified in way that applying transformation $T$ to answer-critic information (\ie causal scene and question) should set off equivariant semantic change in answer space.
    In turn, a cautious formulation of such co-variation should helps the model to pinpoint the 'girl-on-horse' scene as grounding rationale for ``ride''.
    
    \item \textbf{Environmental-invariance.} On ground of the prophet, the answer prediction is invariant against permutation on environment scene, as it does not contribute to the reasoning mechanism or interpretation. 
    Consider the example in Figure \ref{fig:overview} again, since complement as ``landscape'' provide no evidence toward answer ``ride'', its corresponding transformation should reflect a homogeneity in the answer space. The invariance principle epitomizes such assumption by ruling a transformation that is in-vary to answer permutation.
\end{itemize}


%5.overall idea ------------------------------------------------------------------
Aspiring to capture grounding rationale, we formalize a model-agnostic learning framework, Equivariant and Invariant Grounding for Interpretable VideoQA (EGV), 
%
by asking the question ``what and how transformation should the model be equivariant or invariant to?'' 
%
Different from the previous effort that design supervised proxy task for geometric transformation \cite{DBLP:conf/iccv/ChengSM21}, 
% we adopted philosophy of causal intervention and design a saliency-aware temporal mix method for the video input, and impose 
we answer the ``what'' question by adopting the philosophy of causality \cite{pearl2009causal} and configure transformation as causal intervention operation that imposes scene-aware mixup \cite{DBLP:conf/iclr/ZhangCDL18} on the multi-modal input.
%
As for the question of how, we present a unified view of equivariant and invariant principles via the lens of temporal self-supervised learning, where the contrastive counterparts are bred through a disruption on the causal scene, environmental scene as well as vision-language alignment.

% where the contrastive counterparts are bred through a disruption on the causal and environmental scene, respectively.

% implemetation -----------------------------------------------------
In light of this idea, EGV absorbs three modules in addition to the backbone VideoQA model: a grounding indicator, an intervener, and a disruptor. 
%
In particular, the grounding indicator learns to separate the causal scenes as the interpretation and leave the rest as complement. Then the intervener performs a convex combination of two data points with different ratios on their causal and environmental parts. 
%
Noticeably, since mixing environment does not affect the reasoning dynamics, the answer is modified with the same ratio as the causal scene but independent to environmental one. 
%
By capturing the equivariance from the answer to the causal scene and the invariance to environment, the model perceives a faithful interpretation that preserves the predictive mechanism.
%
On top of the intervened video, the disruptor substitutes the complement scene with the stratification sampled from a memory bank (a collection of other training videos) and constitutes the “counterfactual video” as the positive sample.
Likewise, the negative sample is constructed via replacement on the causal scene. 
%
In addition to the visual negatives that ``disrupt'' the causal scene, the disruptor also develops alternatives by disrupting the visual-question coupling, to fortify their pair-wise cohesiveness.
% 
After acquiring anchor representation alongside its contrastive twins, the auxiliary contrastive objective reveals the discriminative representation purely from the scene of interest, thus fostering the robustness of interpretation.

Briefly put, our contributions are: 
\begin{itemize}[leftmargin=*]
    \item We proposed EGV, a model-agnostic VideoQA explainer that captures the intrinsic causal pattern in a self-interpretable manner.
    
    \item We investigate the soundness of grounding rationale by posing the equivariant-invariant principle on visual grounding and realize it via the causal instrument.
    
    \item We justify the superiority of EGV on three popular benchmark datasets (\ie MSVD-QA \cite{DBLP:conf/mm/XuZX0Z0Z17}, MSRVTT-QA \cite{DBLP:conf/mm/XuZX0Z0Z17},  NExT-QA \cite{DBLP:conf/cvpr/XiaoSYC21}) with extensive experiments, where our design outmatches all the state-of-the-art models.
\end{itemize}















==> backup/3_reformulation.tex <==
\section{VideoQA Reformulation}
\label{sec:reformulation}

Discovering the grounding rationale for faithful prediction demands careful inspection of the data generating process. In favor of the causal theory \cite{pearl2016causal}, we review the formation of VideoQA models, then formalize them as a Structure Causal Model (SCM) \cite{alma991011292629705181}  by investigating causality among five variables: the input video $V$ and question $Q$, the causal scene $C$ and its environmental scene $E$, ground-truth answer $A$.

\subsection{Causal Graph of VideoQA}
Scrutinizing the relations among its variables, we abstract the formulation of VideoQA in Figure \ref{fig:scm}a and explain its rationality as follows:

\begin{itemize}[leftmargin=*]
    % \setlength\itemsep{-2pt}
    \item $Q\to C, E \gets V$. Given the semantic of question $Q$,  input video $V$ is composed of a question-critical scene $C$ and $E$--the uninformative part. For example, the video in Figure \ref{fig:overview} is consists of two green clips (\ie $C$) and one blue clip (\ie $E$).
    
    \item $V,Q\to C\to A$. Filtered by question clue, the distilled visual information $C$ contains answer-decisive knowledge that is sufficient to yield answer $A$.
    
    \item $V,Q\to A$. In addition to retrieving $C$, $V$ and $Q$ also deliver a uni-modal message to the classifier. Albeit the underlying bias in some analyses \cite{cadene2019rubi,niu2020counterfactual}, they disclose essential prior statics on the environment. 
    
    \item $E\dashleftarrow\dashrightarrow C$. The dashed arrow sketches adjunctive probabilistic dependencies \cite{reason:Pearl09a} between $C$ and $E$, which is typically rising from selection bias \cite{DBLP:conf/cvpr/TorralbaE11}. For example, the ``landscape'' of the video in Figure.\ref{fig:overview} is frequently collected as a common environment for the ``horse-riding '' scene. 
    
\end{itemize}
\subsection{Beyond ERM}

Inspecting previous efforts, we sketch the SCM for the conventional ERM-guided method in Figure \ref{fig:scm}b.  Probing its causal structure, we investigate the inability of the conventional method in locating the grounding rationale, which shed light on how EGV addresses the problem accordingly.
%
In conventional VideoQA, the $V, Q$ pair is directly paired together to model their interaction and then generates the $A$ as a prediction. Inevitably, such exploitation takes $V$ as a whole and ignores the data generation process, where $C$ and $E$ hold different attribution towards answer semantic. 
%
Driven by ERM, conventional methods blindly capture the statistical correlations between input $(V, Q)$ pairs and answers, while discarding the functional divergence of $C$ and $T$ in the reasoning logic. As a result, such brutal optimization is inept for intrinsic interpretation.

%, make the partition result venerable against environment shift (\ie even a permutation on complement can result in a drastic change on interpretation), and jeopardizes the inept for . 
    
% conventions methods dismiss the formation of $V$ and blindly captures the statistical correlations between input $(V, Q)$ pairs and answers, this makes themselves venerable against environment shift (\ie even a permutation on complement can result in a drastic change on interpretation), and inept for intrinsic interpretation.   
%
Intuitively, a hard split on question-relevant part $C$ naturally serves as the interpretation of the prediction. Following this essence, we present the insight of EGV (Figure \ref{fig:scm}c) by eliminating the effect of environment scene $E$. 
%
In fact, eradicating $E$ from reasoning logic makes $C$ the only component of the input video, thus cutting off  $V \to A$ and emphasizing the impact of $C \to A$.







\begin{figure}[t]
\centering
\includegraphics[scale=0.28]{fig/scm.pdf}
\caption{Causal Graph of VideoQA}
\vspace{-5pt}
\label{fig:scm}
\end{figure}


==> sec/1_intro_new2.tex <==
\section{Introduction}
\label{sec:introduction}


% 1.videoQA overview-----------------------------------------
Video Question Answering (VideoQA) \cite{fan2019heterogeneous} is a keystone in interactive AI, such as vision-language navigation and communication systems.
It aims to answer the natural language question based on the video content.
Striving for the architecture novelty, many studies have been conducted on modeling VideoQA's multi-modal nature, such as fostering the vision-language alignment \cite{jiang2020reasoning,park2021bridge} and revisiting the visual input structure \cite{le2021hierarchical,dang2021hierarchical}.
However, existing VideoQA models usually operate as black boxes, which fail to exhibit the working mechanism behind the predictions and hardly exhibit ``What knowledge should the model use to answer the question about the video?''.
As a result, the black-box nature causes concern for the model's reliability, especially in applications to safety and security.



\begin{figure}[t]
\centering
\includegraphics[scale=0.47]{fig/f1.pdf}
\vspace{-15pt}
\caption{
Illustration of equivariant and invariant grounding.
The causal-equivariant principle (left) asks that the semantic change $T_{\epsilon}$ applied to the causal scene $C$ and question $Q$ should be faithfully reflected in the answer change.
In contrast, the environment-invariant principle (right) outputs the same answer, regardless of changes $T_{\iota}$ on the environment scene $E$.
Here, $f_{\hat{A}}$ maps input to answer space.
% On the left, transformation $T_{\epsilon}$
% Illustration of causal-equivariant and environment-invariant principles.
% On the left, transformations $T_{\epsilon}$ convert the causal scene $C$ and question $Q$ into intervened factors (exemplified as a mixture with the ``man-surfing-in-ocean'' sample) which reflects equivariance in the answer space. On the right, transformation $T_{\iota}$ mixed the two environment scenes and yields an invariant answer. Here, $f_{\hat{A}}$ maps input to answer space.
}
\vspace{-15pt}
\label{fig:overview}
\end{figure}


% 2.problem of interpretable-------------------------------
The concern on the black-box nature calls for better explainability of VideoQA models.
Here we focus on visual-explainability \cite{CSS,DBLP:conf/ijcai/RossHD17}, aiming to reveal ``Which part of the video should the model look at to answer the question?''.
It requires us to find a subset of visual scenes --- rationale --- which are the right reasons for the right answering \cite{DBLP:conf/ijcai/RossHD17}.
Taking Figure \ref{fig:overview} as an example, when answering the question ``What is the girl doing?'', the rationale should focus on the ``girl-riding on-horse'' scene in the first two clips.
Towards this end, existing studies \cite{gao2018motionappearance,DBLP:conf/iccv/Liu0WL21,DBLP:conf/mm/WangG0W21} dwell mainly on the paradigm of \textbf{post-hoc explainability} \cite{LIME,DBLP:conf/iccv/SelvarajuCDVPB17}, which distributes the predictive answer of the target model to the input visual features via an additional explainer method.
They visualize the attention weights or gradient-like signals toward the visual features, and then identify a salient pattern as the rationale.
However, post-hoc explainability has several major limitations:
(1) It fails to make the target model intrinsically interpretable \cite{DBLP:conf/cvpr/YangZQ021,wang2021causal,DBLP:journals/natmi/Rudin19},  only approximating the decision-making process of the model.
As a result, the identified rationale cannot faithfully reveal how the model leverages the multi-modal information.
(2) Such visual inspections are fragile against input perturbations, since some artifacts can be easily captured as explanations instead of genuine knowledge from the data \cite{DBLP:conf/ijcai/LaugelLMRD19,slack2020fooling,heo2019fooling,ghorbani2019interpretation}.




% 3.partition the video to get interpretation ------------
The limitations of post-hoc explainability inspire us to explore the paradigm of \textbf{intrinsic interpretability} \cite{ghorbani2019interpretation,DBLP:journals/natmi/Rudin19}, which embeds a rationalization module into the model to make the decision-making process transparent.
Surprisingly, the intrinsic interpretability of VideoQA models is until-now lacking.
To fill the void, we draw on \textbf{causal theory} \cite{pearl2016causal,pearl2009causal} to formulate the interpretability task as disclosing ``Which part of the video is critical/causal to answering the question?''.
Concretely, we aim to identify the causal component of input video on-the-fly, which holds the question-response information and filters out the question-irrelevant cues.
Following this essence, one straightforward realization is to ground the input video into two segments:
(1) \textbf{causal scene}, which retains the question-critical visual content and sufficiently approaches the answer, thus naturally serving as the rationale;
and (2) \textbf{environment scene}, which holds the question-irrelevant visual content and can be seen as the rationale's complement.



% 4.euiqvariant and invariant -------------------------------
% 要突出的是grounding，title中是Equivariant and invariant grounding，所以要让这些关键词尽早的出现。
% 这个例子融入到下面的Causal-Equivariance和Environmental-Invariance中去。
%
However, discovering causal scene without the supervision of ground-truth rationale is challenging.
With a causal look at the reasoning process (\cf Section \ref{sec:causal-view}), we argue that the crux of intrinsic interpretability is to amplify the connection between the causal scene and the answer, while blocking the non-causal effect of the environment scene.
Following this line, we propose two principles to guide the grounding of the rationale:
\begin{itemize}[leftmargin=*]
    \item \textbf{Causal-Equivariance.}
    By ``equivariance'', we mean that answering should be sensitive to the semantic changes on the causal scene and question (termed E-intervention), \eg any change on the causal scene and question should be faithfully reflected on the predicted answer. For example, in Figure \ref{fig:overview}, the ``girl-riding on-horse'' and ``man-surfing in-ocean'' scenes are the oracle rationales of ``What is the girl doing?'' and ``What is the man doing?'', respectively. The intervention applied on the input (\ie mixing the ``girl-riding on-horse'' and ``man-surfing in-ocean'' scene, and combining two questions as ``What is the girl doing? What is the man doing?'') should set off an equivariant change in the answer (\ie changing from ``Ride'' to ``Ride+Surf'').
    
    
    
    \item \textbf{Environment-Invariance.}
    By ``invariance'', we mean that answering should be insensitive to the changes in the environment scene (termed I-intervention), conditioning on the causal scene and question.
    Considering Figure \ref{fig:overview} again, the intervention applied to the environment (\ie mixing the ``meadow'' and ``ocean'' scenes) implies no impact towards answering ``What is the girl doing?'', reflecting a homogeneity in the answer space.
\end{itemize}


%5.overall idea ------------------------------------------------------------------
% Aspiring to capture grounding rationale, we formalize a model-agnostic learning framework, Equivariant and Invariant Grounding for Interpretable VideoQA (EIV), 
% %
% by asking the question ``what and how transformation should the model be equivariant or invariant to?'' 
% %
% Different from the previous effort that design supervised proxy task for geometric transformation \cite{DBLP:conf/iccv/ChengSM21}, 
% % we adopted philosophy of causal intervention and design a saliency-aware temporal mix method for the video input, and impose 
% we answer the ``what'' question by adopting the philosophy of causality \cite{pearl2009causal} and configure transformation as causal intervention operation that imposes scene-aware mixup \cite{DBLP:conf/iclr/ZhangCDL18} on the multi-modal input.
% %
% As for the question of how, we present a unified view of equivariant and invariant principles via the lens of temporal self-supervised learning, where the contrastive counterparts are bred through a disruption on the causal scene, environment scene as well as vision-language alignment.

% where the contrastive counterparts are bred through a disruption on the causal and environment scene, respectively.

% implemetation ----------------------------------------------
% 这一段的写作逻辑应该是如何实现equivariant、invariant principles的；可以不用follow IGV的写法；

% 可以这么组织：
% 一句话介绍三个modules；
% 然后如何用这三个modules来实现两个principle的：首先用grouidng indicator去roughly partition videos into two parts：causal and environmental scenes；然后基于这两部分引入causal-equivariance：利用interventer对于causal scenes做interventions，期望answer部分产生相对应的变化；利用interventer对于environmental scenes做interventions，期待这部分不会对于answering产生影响。

To impose these two principles for intrinsic interpretability, we propose a new framework, \underline{E}quivariant and \underline{I}nvariant \underline{G}rounding for Interpretable \underline{V}ideoQA (\textbf{EIGV}).
EIGV equips the VideoQA backbone model with three additional modules:
a grounding indicator, an intervener, and a disruptor.
First, the grounding indicator learns to attend the causal scene based on the input question, while leaving the rest as the environment.
% However, this grounding only roughly estimates the oracle partition of causal and environment scenes.
Then, the intervener parameterizes the proposed principles to guide the grounding.
Specifically, towards the causal-equivariance principle, it conducts the E-intervention on the causal scene and question --- that is, mix them with the counterparts from another video-question pair --- and encourages the predictive answer to be anticipated accordingly.
Towards the environment-invariance principle, when leaving the causal scene and question untouched, it applies the I-intervention on the environment --- that is, mix it with the environmental stratification of a memory bank --- and enforces the predictive answer to be invariant.
Moreover, we build an unified sight of two principles via the lens of contrastive learning.
Concretely, on top of each intervened video-question pair, the disruptor constructs the positive views by disrupting the environment scene randomly, while creating the negative views by substituting the causal scene with random scenes.
Training with these two principles allows the backbone model to distinguish the causal scene from the environmental cues, and hinge on the critical visual-linguistic alignment. 


Briefly put, our contributions are: 
\begin{itemize}[leftmargin=*]
    \item We propose EIGV, a model-agnostic VideoQA framework that distills the causal visual-linguistic alignment to generate answers in a self-interpretable manner.
    
    \item We investigate the soundness of grounding rationale by posing the equivariant-invariant principle on visual grounding.
    
    \item We justify the superiority of EIGV on three popular benchmark datasets (\ie MSVD-QA \cite{DBLP:conf/mm/XuZX0Z0Z17}, MSRVTT-QA \cite{DBLP:conf/mm/XuZX0Z0Z17},  NExT-QA \cite{DBLP:conf/cvpr/XiaoSYC21}) with extensive experiments, where our design outmatches the state-of-the-art models. Moreover, our EIGV is a model-agnostic framework that can be applied to different VideoQA models. 
\end{itemize}















==> sec/8_limits.tex <==
\section{Limitation and Complexity}
\label{section:limits}
\lyc{In addition to the technical advantages, we discuss possible limits of the current design. Unlike some SoTAs that utilize object-level features (\eg HOSTR \cite{dang2021hierarchical} and PGAT \cite{DBLP:conf/mm/PengYBW21}), EIVG merely takes advantage of clip-level representation. Although the architecture of the backbone model is beyond the scope of this work, we anticipate that a fine-grained interpretation at the entity level will strengthen the current EIGV design.
% 2) Current intervention strategy can possibly threaten the causal prediction by introducing context with new shortcuts. Since the scene intervener sample context stratification in a random manner, there is a slight chance to draw an undesired substitute that nested with strong static relation towards  a wrong answer, thus inducing a false prediction.
In terms of complexity, we run all experiments on NVIDIA Tesla V100 GPU, where our algorithm matched equally with the corresponding baseline.  For comparison, the backbone MSPAN model is trained for 1.5 hours till convergence on NExT-QA, whereas EIGV 
takes 1.6 hours.
}
